Understanding Multi-Granularity for Open-Vocabulary Part Segmentation

Open-vocabulary part segmentation (OVPS) is an emerging research area focused on segmenting fine-grained entities using diverse and previously unseen vocabularies. Our study highlights the inherent complexities of part segmentation due to intricate boundaries and diverse granularity, reflecting the knowledge-based nature of part identification. To address these challenges, we propose PartCLIPSeg, a novel framework utilizing generalized parts and object-level contexts to mitigate the lack of generalization in fine-grained parts. PartCLIPSeg integrates competitive part relationships and attention control, alleviating ambiguous boundaries and underrepresented parts. Experimental results demonstrate that PartCLIPSeg outperforms existing state-of-the-art OVPS methods, offering refined segmentation and an advanced understanding of part relationships within images. Through extensive experiments, our model demonstrated a significant improvement over the state-of-the-art models on the Pascal-Part-116, ADE20K-Part-234, and PartImageNet datasets.

==> sections/07_rebuttal.tex <==





% TODO: 

\newpage
\newpage

\appendix

\startcontents[rebuttal] % 'rebuttal' prefix


\setcounter{section}{0}   
\renewcommand{\thetable}{R\arabic{table}}
\setcounter{table}{0}   
\renewcommand{\thefigure}{R\arabic{figure}}
\setcounter{figure}{0}  
\renewcommand{\theequation}{R\arabic{equation}}
\setcounter{equation}{0}  

% \vspace{-2.5em}

% \renewcommand\contentsname{Rebuttal Material}



\clearpage
\renewcommand\contentsname{\small Response Materials}
% \renewcommand\contentsname{Response Materials for Reviewers' Comments on Paper \#10487}
\addtocontents{toc}{\protect\setcounter{tocdepth}{2}}
\tableofcontents 


% \vspace{-2.5em}
\vspace{-2.2em}




% CLIPSeg (CVPR 2022.06)
% ZSSeg (ECCV 2022.10)
% VLPart (ICCV 2023.10)
% CATSeg (CVPR 2024.06)
% OV-PARTS (NeurIPS 2023.12)

% \begin{table}[ht]
\begin{table}[ht]
    \captionsetup{type=table,font=scriptsize}
    \caption{Comparison of zero-shot performance with state-of-the-art methods on Pascal-Part-116.}
    \label{tab_rebuttal:main_pascal}
    \centering
    \begin{small}
    \scalebox{0.85} {
        
        \begin{threeparttable}
        \begin{tabular}{@{}llcccccccccc@{}}
            \toprule
            \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{1}{c}{\multirow{2}{*}{Backbone}} & \multicolumn{3}{c}{Pred-All} & \multicolumn{3}{c}{Oracle-Obj} \\ \cmidrule(l){3-5} \cmidrule(l){6-8} 
             &  & Seen & Unseen & Harmonic & Seen & Unseen & Harmonic  \\ \midrule
            \rowcolor{blue!25}
            \multirow{1}{*}{\cellcolor{cyan}VLPart \cite{sun2023going_VLPart}} & ResNet-50  & 36.65 & 10.19 & 15.95 & 42.61 & 18.70 & 25.99 \\
            CLIPSeg \cite{luddecke2022image_CLIPSeg,wei2024ov_OV_PARTS} & ViT-B/16 & 44.90 & 18.80 & 26.50 & 46.50 & {28.41} & {35.27} \\
            \midrule
            PartCLIPSeg (ours) & ViT-B/16 & 44.37$_{\pm0.43}$ & {27.29}$_{\pm0.21}$ & \textbf{33.79}$_{\pm0.08}$ & 50.02$_{\pm0.50}$ & {31.67}$_{\pm0.27}$ & \textbf{38.79}$_{\pm0.11}$ \\ 
            \bottomrule
        \end{tabular}
        \end{threeparttable}
    }
\end{small}
% \vspace{-1.5em}
\vspace{-1.0em}
\end{table}





\begin{minipage}{0.35\textwidth}
    \small
    \centering
    \captionsetup{type=figure,font=scriptsize}
    \captionof{table}{Ablation Study: Impact of $\lambda_{\texttt{obj}}$, $\lambda_{\texttt{part}}$, and , $\mathcal{L}_{\texttt{sep}} + \mathcal{L}_{\texttt{enh}}$ on Pascal-Part-116 (Oracle-Obj)}
    \vspace{-0.5 em}
\vfill
    \label{table_rebuttal:ablation_sep_and_enh}
    \scalebox{0.65}
    {
    \begin{tabular}{@{}ccc  ccc@{}}
        \toprule
        $\lambda_{\texttt{obj}}$ & $\lambda_{\texttt{part}}$ & $\mathcal{L}_{\texttt{sep}} + \mathcal{L}_{\texttt{enh}}$ & Seen & Unseen & Harmonic \\ \midrule
        0.0  &  0.0  &  \yesmark   &  48.36  &  29.42  &  36.58  \\
        1.0  &  0.0  &  \yesmark   &  48.61  &  31.28  &  38.07  \\
        0.0  &  1.0  &  \yesmark   &  48.94  &  31.68  &  38.46  \\
        1.0  &  1.0  &  \yesmark   & {50.02} & {31.67} & \textbf{38.79} \\
        1.0  &  1.0  &  \nomark    & {49.09} & {31.26} & {38.20} \\
        % \midrule
        \bottomrule
    \end{tabular}
    }
% \vspace{-1.5em}
\end{minipage}%
\hfill
\begin{minipage}{0.3\textwidth}
    \small
    \centering
\vfill
    % \captionsetup{hypcap=false,font=scriptsize}
    \captionsetup{hypcap=false,font=scriptsize}
    \captionof{table}{Performance along boundaries: Mean boundary IoU ($\uparrow$) on Pascal-Part-116 (Oracle-Obj)}
    \vspace{-0.5 em}
    \captionsetup{font=scriptsize}
    \label{tab_rebuttal:boundary_iou}
    \begin{small}
    \scalebox{0.70}{
        \begin{tabular}{@{}lcccccccccc@{}}
            \toprule
            \multicolumn{1}{c}{\multirow{1}{*}{Method}} & Seen & Unseen & Harmonic  \\
            \midrule
            ZSSeg        & 33.01  & 26.76  & 29.56 \\
            CAT-Seg      & 34.17  & 30.14  & 32.03 \\
            CLIPSeg      & 34.67  & 32.20  & 33.39 \\
            PartCLIPSeg  & 36.15  & 39.07  & \textbf{37.55} \\
            \bottomrule
        \end{tabular}
    }
    \end{small}
\end{minipage}
\hfill
\begin{minipage}{0.3\textwidth}
    \small
    \centering
\vfill
    \captionsetup{hypcap=false,font=scriptsize}
    \captionof{table}{Computational resources ($\downarrow$) on Pascal-Part-116 \\(Batch: 8)}
    \vspace{-0.5 em}
    \captionsetup{font=scriptsize}
    \label{tab_rebuttal:computational_resource}
    \begin{small}
    \scalebox{0.70} {
        \begin{tabular}{@{}lcc@{}}
            \toprule
            \multicolumn{1}{c}{Method} & \multicolumn{1}{c}{Params} & \multicolumn{1}{c}{Memory}  \\
            \midrule
            ZSSeg		& 191.6 M		& 11.1 G \\
            CAT-Seg		& 180.6 M		& 29.0 G \\
            CLIPSeg		& 151.7 M		& 25.5 G \\
            PartCLIPSeg	& 152.4 M		& 24.4 G \\
            \bottomrule
        \end{tabular}
    }
    \end{small}
\end{minipage}

% -------------------------------------------------------------------------






\begin{minipage}{\textwidth}
    \centering
    \begin{minipage}{0.70\textwidth}
        \centering
        \begin{minipage}{.32\textwidth}
            \centering
            \includegraphics[height=2.5cm, width=3.5cm]{assets/intro_CLIPSeg_2010_001016.png}
        \end{minipage}\hfill
        \begin{minipage}{.32\textwidth}
            \centering
            \includegraphics[height=2.5cm, width=3.5cm]{assets/intro_CLIPSeg_2008_004704.png}
        \end{minipage}\hfill
        \begin{minipage}{.32\textwidth}
            \centering
            \includegraphics[height=2.5cm, width=3.5cm]{assets/intro_CLIPSeg_2010_001016.png}
        \end{minipage}
        % Second row
        \begin{minipage}{.32\textwidth}
            \centering
            \includegraphics[height=2.5cm, width=3.5cm]{assets/rebuttal/vis_challenge/2008_002904.jpg}
            \vspace{-0.2em}
            \scalebox{0.65}{(a) Lack of generalization}
        \end{minipage}\hfill
        \begin{minipage}{.32\textwidth}
            \centering
            \includegraphics[height=2.5cm, width=3.5cm]{assets/rebuttal/vis_challenge/2008_004704.jpg}
            \vspace{-0.2em}
            \scalebox{0.65}{(b) Ambiguous boundaries}
        \end{minipage}\hfill
        \begin{minipage}{.32\textwidth}
            \centering
            \includegraphics[height=2.5cm, width=3.5cm]{assets/rebuttal/vis_challenge/2010_001016.jpg}
            \vspace{-0.2em}
            \scalebox{0.65}{(c) Underrepresented part}
        \end{minipage}
        \label{fig_rebuttal:challenges_in_ovps_figure}
        \vspace{-1.5em}
        \captionsetup{font=scriptsize, skip=2em}
        \captionof{figure}{Three challenges of existing OVPS methods (VLPart, CLIPSeg) in the upper row and impact of PartCLIPSeg in the bottom row in the prediction of seen (aeroplane) and unseen (dog, bird) categories. (misclassification of sheep's ear disappeared, the boundaries of aeroplane's tail and wing become more accurate, underrepresented parts such as bird's tail and beak detected)}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{assets/rebuttal/2010_004226_sep_only.pdf}
        \includegraphics[width=\textwidth]{assets/rebuttal/2010_004226_sep_enh.pdf}
        \captionsetup{font=scriptsize}
        \vspace{-1.2em}
        \captionof{figure}{
            Comparison of results using only $\mathcal{L}_{\texttt{sep}}$ (top) with both $\mathcal{L}_{\texttt{sep}}$ and $\mathcal{L}_{\texttt{enh}}$ (bottom). The heatmap illustrates attention activation for the sheep's neck class.
        }

    \end{minipage}
\end{minipage}











% ----------------------------------------------------------------------------
\begin{figure}[ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.99\textwidth]{assets/rebuttal/qualitative_vlpart_with_GT.png}
    \vspace{-0.6em}
    \captionsetup{type=figure,font=scriptsize}
    \captionof{figure}{
        GT (top), VLPart (middle), PartCLIPSeg (bottom) in Pred-All setting. While both VLPart and PartCLIPSeg perform well on seen classes like cat and airplane, PartCLIPSeg notably excels with novel classes such as dog, bird, sheep, and car.
    }
    \label{fig_rebuttal:overview}
    % \vspace{-0.5em}
\end{figure}
% ----------------------------------------------------------------------------









\begin{figure}[ht]
    \centering
    \vspace{-1.4em}
    \begin{minipage}[t]{0.67\textwidth}
        \centering
        \includegraphics[height=4cm]{assets/rebuttal/part_size_plot.png}
        \captionsetup{type=figure,font=scriptsize}
        \caption{
            Average size ratio (left) and comparison of PartCLIPSeg with CLIPSeg on small object-specific parts (size < 0.2) in Pascal-Part-116. Green and red indicate categories where PartCLIPSeg and CLIPSeg outperform, respectively. Yellow classes are selected from Table 6.
        }
        \label{fig:image1}
    \end{minipage}
    \hspace{0.5em}
    \begin{minipage}[t]{0.27\textwidth}
        \centering
        \includegraphics[height=4cm]{assets/supplementary/dataset_object_size_distribution_plot.png}
        \vspace{-1.1em}
        \captionsetup{type=figure,font=scriptsize}
        \captionof{figure}{
            Distribution of object size ratios across datasets.
        }
        \label{fig:image2}
    \end{minipage}
\end{figure}








